FigCaps-HF: A Figure-to-Caption Generative Framework and Benchmark with Human Feedback

Captions are crucial for understanding scientific visualizations and documents. Existing captioning methods for scientific figures rely on figure-caption pairs extracted from documents for training, many of which fall short with respect to metrics like helpfulness, explainability, and visual-descriptiveness [15] leading to generated captions being misaligned with reader preferences. To enable the generation of high-quality figure captions, we introduce FigCaps-HF a new framework for figure-caption generation that can incorporate domain expert feedback in generating captions optimized for reader preferences. Our framework comprises of 1) an automatic method for evaluating quality of figure-caption pairs, 2) a novel reinforcement learning with human feedback (RLHF) method to optimize a generative figure-to-caption model for reader preferences. We demonstrate the effectiveness of our simple learning framework by improving performance over standard fine-tuning across different types of models. In particular, when using BLIP as the base model, our RLHF framework achieves a mean gain of 35.7%, 16.9%, and 9% in ROUGE, BLEU, and Meteor, respectively. Finally, we release a large-scale benchmark dataset with human feedback on figure-caption pairs to enable further evaluation and development of RLHF techniques for this problem.

==> model_parameters.tex <==

% \begin{table}
% \centering
% \caption{
% Model hyperparameter details 
% \todo{FIX!! actually add hyperparam details}
% }
% \label{table:model-parameters}
% \renewcommand{\arraystretch}{1.15} 
% % \setlength{\tabcolsep}{3.9pt} 
% \small

% \begin{tabularx}{1.0\linewidth}{l l c HH HH Hc cH Hccc}
% \toprule
% &
% \textsc{Model} &  
% \textbf{\#Params} & 
% \textbf{Generation Strategy} &
% R@1 & \sc Norm. & %R@1 & 
% R@2 & \sc Norm. & %R@2 & 
% % \sc Norm. & %R@L &
% \textbf{Generation} &
% \textbf{lr} &
% \textbf{Epochs} &
% \\ \midrule

% \multirow{1}{*}{\textsc{ocr-only}}
% & \textbf{Pegasus}~\cite{zhang2020pegasus} & 0.27B &&&&&& TODO \\ 

% \midrule
% \multirow{4}{*}{\textsc{Figure-Only}}
% & \textbf{TrOCR}~\cite{li2021trocr} & 0.23B &&&&&& TODO\\ 
% & \textbf{BEiT+GPT2}~\cite{} & 0.24B &&&&&& Greedy \\ 
% & \textbf{ViT\cite{dosovitskiy2020vit} + RoBERTA\cite{liu2019roberta}} & 0.23B &&&&&& TODO\\ 
% & \textbf{ViT\cite{dosovitskiy2020vit} + GPT2} & 0.24B &&&&&& Greedy \\ 
% \midrule
% \multirow{5}{*}{\textsc{Figure-Caption}}
% & \textbf{PromptCap}~\cite{hu2022promptcap} & 0.47B &&&&&& TODO \\ 
% & \textbf{Flamingo}~\cite{alayrac2022flamingo} & 1.14B &&&&&& Greedy  \\ 
% & \textbf{GIT~\cite{wang2022git}} & 0.17B &&&&&& Greedy \\
% & \textbf{BLIP \cite{li2022blip}} & 0.25B &&&&&& Nucleus  \\ 
% & \textbf{CLIPCap} & 0.15B &&&&&& Greedy  \\ 
% \midrule
% \multirow{4}{*}{\textsc{rlhf}}
% % \multirow{4}{*}{\textsc{Feedback-Prompt (Prepend)}}
% % PREPENDED & 'good' prompt during inference.
% & \textbf{Ours-BLIP-RLHF} & 0.25B &&&&&& Nucleus  \\ 
% % & \textbf{Ours-CLIPCap-RLHF} & 0.15B &&&&&& TODO \\ 
% & \textbf{Ours-ViT+GPT2-RLHF} & 0.24B &&&&&& Greedy  \\  


% \bottomrule
% \end{tabularx}
% \end{table}

==> table-benchmark-data-stats.tex <==

% train, validate, test
% 106,834 	13,354 	13,355
% train=106,834 	validate=13,354 	test=13,355
\begin{table}[t]
\centering
% \vspace{-6mm}
\renewcommand{\arraystretch}{1.15} 
% \setlength{\tabcolsep}{3.9pt} 
\small
% \footnotesize
% \scriptsize
% \begin{tabularx}{1.0\linewidth}{l @{}c HH HH cc cc cccc}
\begin{tabularx}{1.0\linewidth}{l @{}c l c cc Hc c H HH HH}
\toprule
% & 
% % \multirow{2}{*}{\sc \# Trainable} 
% &
% \multicolumn{2}{c}{ROUGE-1} & 
% \multicolumn{2}{c}{\sc ROUGE-2} &
% % &&&&
% \multicolumn{2}{c}{\sc ROUGE-L} & \\
% \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}

% INFERRED HUMAN FEEDBACK
% | Category  | Median    | Mean      | Standard Deviation | Minimum   | 25th Percentile | 75th Percentile | Maximum   |
% |-----------|-----------|-----------|--------------------|-----------|----------------|----------------|-----------|
% | Helpfulness | 2.887949 | 2.891968 | 1.067641           | -1.271212 | 2.167202       | 3.610363       | 7.605054 |
% | Takeaway  | 1.948700 | 2.058931 | 1.028708           | -1.061640 | 1.330719       | 2.660354       | 8.144583 |
% | Visual    | 1.913612 | 2.024573 | 1.010477           | -1.233484 | 1.307569       | 2.625947       | 7.971579 |
% | OCR       | 3.882775 | 3.840144 | 0.828866           | 0.017950  | 3.319476       | 4.406052       | 7.505501 |

% & \textbf{\# Fig-Caption} & \\
% & \textbf{Pairs} & 
& \textbf{\# Fig-Caption Pairs} &
\textbf{Human Feedback}  & \textbf{Median}    & \textbf{Mean}      & \textbf{Std} & \textbf{Min}   & \textbf{Q1} & \textbf{Q3} & \textbf{Max}   &\\
\midrule


\multirow{3}{*}{\textsc{Actual}} % HF (400)}}
& \multirow{4}{*}{\textbf{438}}
% ACTUAL HUMAN FEEDBACK
	   % Median	Mean	Std	Min	25%	50%	75%	Max
&  \textbf{Helpfulness}	 & 3	 & 3.01	 & 1.19	 & 1	 & 2	 & 3		 & 5\\
 \multirow{3}{*}{\textsc{Human Feedback}}
& & \textbf{Takeaway}	 & 	2 & 	2.16 & 	1.22 & 	1	 & 1	 & 2 & 		5\\
& & \textbf{Visual}	&	2	 & 2.11	 & 1.08	 & 1 & 	1	 & 2	 &  	5\\
& & \textbf{OCR}	 & 	4	 & 3.83 & 	0.80 & 	1	 & 4 & 	4	 &  	5\\

\midrule
% train=106,834 	validate=13,354 	test=13,355
\multirow{3}{*}{\textsc{Predicted}} % (100K+)}}
& \multirow{4}{*}{\textbf{106,834}} % (100K+)}}
& \textbf{Helpfulness} & 2.89 & 2.89 & 1.07           & -1.271212 & 2.17       & 3.61       & 7.605054 &\\
\multirow{3}{*}{\textsc{Human Feedback}}
&& \textbf{Takeaway}  & 1.95 & 2.06 & 1.03           & -1.061640 & 1.33       & 2.66       & 8.144583 &\\
&& \textbf{Visual}    & 1.91 & 2.02 & 1.01           & -1.233484 & 1.31       & 2.63       & 7.971579 &\\
&& \textbf{OCR}       & 3.88 & 3.84 & 0.83           & 0.017950  & 3.32      & 4.41       & 7.505501 &\\


\bottomrule
\end{tabularx}
\caption{%
Summary of our benchmark dataset for figure-caption generative models with RLHF.
}

\label{table:benchmark-data-stats}
% \vspace{-2mm}
% \vspace{-2mm}
\end{table}


==> table-results-HF-filtering.tex <==


\begin{table}
\centering
\caption{%
Results with filtering via predicted human feedback.
% Comparison with state-of-the-art methods. 
% \todo{add more context, keep it short}
% \todo{Please make sure all methods are listed correctly, caption-only, figure-only, figure-caption}
% \ryan{Is BLEU score correct for TrOCR? 
% Also, I think these numbers need to be multipled by 100 (See BLIP and other papers)?}
% For all the metrics, higher values are better ($\uparrow$).
% BLEU=BLEU@4 (add somewhere in paper to clarify)
}
\label{table:results-comparison-filtering}
\renewcommand{\arraystretch}{1.15} 
% \setlength{\tabcolsep}{3.9pt} 
\small
% \footnotesize
% \scriptsize
% \begin{tabularx}{1.0\linewidth}{l @{}c HH HH cc cc cccc}
\begin{tabularx}{0.8\linewidth}{l l H HH HH Hc cH Hccc}
\toprule
% & 
% % \multirow{2}{*}{\sc \# Trainable} 
% &
% \multicolumn{2}{c}{ROUGE-1} & 
% \multicolumn{2}{c}{\sc ROUGE-2} &
% % &&&&
% \multicolumn{2}{c}{\sc ROUGE-L} & \\
% \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
&
\textsc{Model} & 
% \textsc{Parameters} & 
\textbf{\#Params} & 
R@1 & \sc Norm. & %R@1 & 
R@2 & \sc Norm. & %R@2 & 
R@L & 
% \sc Norm. & %R@L &
\textbf{ROUGE-L} &
\textbf{BLEU} & 
\textbf{CIDEr} & 
\textbf{SPICE} &
\textbf{METEOR} &
\\ \midrule


% \multirow{1}{*}{\textsc{OCR-Only}}
% & \textbf{Pegasus TODO (pretrained)}~\cite{zhang2020pegasus} & 0.27B & 0 & 0 & 0 & 0 & 0 & 0.026 & 7.8e-5 & 0.01 & 0.0 & 0.042 \\ 
% % & \textbf{Pegasus (pretrained)}~\cite{zhang2020pegasus} & 0.27B & 0 & 0 & 0 & 0 & 0 & 0.435 & 0.271 & 1.741 & 0 & 0.413 \\ 

% \midrule
% \multirow{1}{*}{\textsc{Figure-Only}}
% & \textbf{TrOCR}~\cite{li2021trocr} & 0.23B & 0 & 0 & 0 & 0 & 0 & 0.025 & 0.0 & 0.001 & 0.0 & 0.018 \\ 
% & \textbf{ViT\cite{dosovitskiy2020vit} + RoBERTA\cite{liu2019roberta}} & 0.23B & 0 & 0. & 0 & 0 & 0 & 0.140 & 0.005 & 0.059 & 0 & 0.121\\ 
% & \textbf{ViT\cite{dosovitskiy2020vit} + GPT2} & 0.24B & 0 & 0 & 0 & 0 & 0 & 0.142 & 0.006 & 0.061 & 0 & 0.126 \\ 

% & \textbf{BEiT+GPT2}~\cite{} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.142 & 0.005 & 0.054  & 0 & 0.124 \\ 
% & \textbf{BEiT+GPT2 with BLIP Filter dataset (50 percentile)} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.127 & 0.002 & 0.000  & 0 & 0.111 \\ 
% & \textbf{BEiT+GPT2 with MCSE Filtered dataset (50\% @ 5 epochs)} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.132 & 0.003 & 0.054  & 0.0 & 0.121 \\ 
% & \textbf{BEiT+GPT2 with MCSE Filtered dataset (50\% @ 10 epochs)} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.135 & 0.016 & 0.054  & 0.0 & 0.125 \\ 


& \textbf{BEiT+GPT2} & 0.24B & 0 & 0 & 0 & 0 & 0 &  \textbf{0.142} & {0.005} & 0.054  & 0 & 0.124 \\ 
\midrule
& \textbf{BEiT+GPT2 with BLIP Filtering} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.127 & {0.002} & 0.000  & 0 & 0.111 \\ 
% & \textbf{BEiT+GPT2 w/ MCSE Filtered dataset (50\% @ 5 epochs)} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.132 & 0.003 & 0.054  & 0.0 & 0.121 \\ 
& \textbf{BEiT+GPT2 with MCSE Filtering} & 0.24B & 0 & 0 & 0 & 0 & 0 &  0.135 & \textbf{0.016} & 0.054  & 0.0 & \textbf{0.125} \\ 

% \midrule
% \multirow{5}{*}{\textsc{Figure-Caption}}
% % https://huggingface.co/vqascore/promptcap-coco-vqa (check if another version exists)
% % & \textbf{PromptCap(0-shot)}~\cite{hu2022promptcap} & 0.47B & 0 & 0 & 0 & 0 & 0 & 0.130 & 0.004 & 0.121 & 0 & 0.082\\ 
% & \textbf{PromptCap}~\cite{hu2022promptcap} & 0.47B & 0 & 0 & 0 & 0 & 0 & 0.130 & 0.004 & 0.121 & 0 & 0.082\\ 


% % https://huggingface.co/dhansmair/flamingo-mini
% & \textbf{Flamingo}~\cite{alayrac2022flamingo} & 1.14B & 0 & 0 & 0 & 0 & 0 & 0.0865 & 0.0002 & 0.0152 & 0 & 0.0459\\ 
% % & \textbf{Flamingo-mini}~\cite{alayrac2022flamingo} & 1.14B & 0 & 0 & 0 & 0 & 0 & 0.0865 & 0.0002 & 0.0152 & 0 & 0.0459\\ 
% % % https://huggingface.co/allenai/scibert_scivocab_uncased
% % & \textbf{SciBERT}~\cite{zhang2021vinvl} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0\\ 

% & \textbf{GIT~\cite{wang2022git}} & 0.17B & 0 & 0 & 0 & 0 & 0 & 0.119 & 0.0018 & 4.8e-7 & 0 & 0.0906 \\
% % & \textbf{GIT (fine-tuned)~\cite{wang2022git}} & 0.17B & 0 & 0 & 0 & 0 & 0 & 0.119 & 0.0018 & 4.8e-7 & 0 & 0.0906 \\
% % & \textbf{GIT (pretrained)\cite{wang2022git}} & 0.17B & 0 & 0 & 0 & 0 & 0 & 0.106 & 0.001 & 0.0179 & 0 & 0.057 \\ 

% & \textbf{BLIP \cite{li2022blip}} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.13 & 0.0143 & TODO & 0 & 0.132 \\ 

% % & \textbf{BLIP \cite{li2022blip}} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.169 & 0.027 & 0.17 & 0 & 0.139 \\ 

% % & \textbf{BLIP \cite{li2022blip}+OCR} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.169 & 0.028 & 0.169 & 0 & 0.140 \\ 
% \midrule
% % OCR-caption contrastive loss + others fine-tuned as well, inference uses only figure+OCR
% % OCR-caption contrastive loss + others fine-tuned as well, inference uses only figure
% % & \textbf{Ours-OCR-Caption-CLoss+others fine-tuned} & 0.27B & 0 & 0 & 0 & 0 & 0 & 0.116 & 0.0008 & TODO &  0 & 0.09 \\ 
% % & \textbf{Ours-OCR-Caption-CLoss+others fine-tuned (Epoch 2)} & 0.27B & 0 & 0 & 0 & 0 & 0 & 0.112 & 0.008 & TODO &  0 & 0.11267 \\ 
% & \textbf{Ours-BLIP-RLHF (MLP) } & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.212 & 0.034 & TODO &  0 & 0.18 \\ 
% & \textbf{Ours-VIT-GPT2-RLHF (MLP) } & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.151 & 0.007 & TODO &  0 & 0.14 \\ 
% % & \textbf{Ours-BLIP-RLHF (MLPRegressor Scoring) } & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.212 & 0.034 & TODO &  0 & 0.18 \\ 
% % & \textbf{Ours-VIT-GPT2-RLHF (MLPRegressor Scoring) } & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.151 & 0.007 & TODO &  0 & 0.14 \\ 
% % OCR-caption contrastive loss + language fine-tuned (same as BLIP+OCR), inference uses only figure
% % & \textbf{Ours-OCR-Caption-CLoss} & 0.27B & 0 & 0 & 0 & 0 & 0 & 0.10794 & 0.000855 & TODO & 0 &  0.09758 \\ 
% % OCR-caption contrastive loss + language fine-tuned (same as BLIP+OCR), inference uses only figure+OCR
% % & \textbf{Ours-OCR-Caption-CLoss} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 
% % & \textbf{Ours} & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\ 

\bottomrule
\end{tabularx}
\end{table}


==> table-results-multiHF.tex <==


\begin{table}[h!]
\centering
\vspace{4mm}
% \vspace{-2mm}
% \caption{%
% Results with multi-labeled human feedback.
% % \todo{Fix table captions, for NeurIPS I think need to be on top of table, not bottom}
% }
\renewcommand{\arraystretch}{1.15} 
% \setlength{\tabcolsep}{3.9pt} 
\small
% \footnotesize
% \scriptsize
% \begin{tabularx}{1.0\linewidth}{l @{}c HH HH cc cc cccc}
\begin{tabularx}{0.8\linewidth}{l l H HH HH Hc cH Hccc}
\toprule
% & 
% % \multirow{2}{*}{\sc \# Trainable} 
% &
% \multicolumn{2}{c}{ROUGE-1} & 
% \multicolumn{2}{c}{\sc ROUGE-2} &
% % &&&&
% \multicolumn{2}{c}{\sc ROUGE-L} & \\
% \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
&
\textsc{Model} & 
% \textsc{Parameters} & 
\textbf{\#Params} & 
R@1 & \sc Norm. & %R@1 & 
R@2 & \sc Norm. & %R@2 & 
R@L & 
% \sc Norm. & %R@L &
\textbf{ROUGE-L} &
\textbf{BLEU} & 
\textbf{CIDEr} & 
\textbf{SPICE} &
\textbf{METEOR} &
\\ \midrule

% & \textbf{BLIP with Multi-labeled feedback(10 epochs multi label)} 
% & \textbf{BLIP with Multi-labeled feedback(10 epochs multi label)} 
& \textbf{Binary Feedback} 
& 0.25B & 0 & 0 & 0 & 0 & 0 & 0.152 & 0.019 & TODO &  0 & 0.145 \\ 

& \textbf{Multi-label Feedback}
& 0.25B & 0 & 0 & 0 & 0 & 0 &   0.153 &  \textbf{0.022} & 0.000  & 0 & \textbf{0.151} \\ 
% & \textbf{BLIP with Multi-labeled feedback (5 epoch binary +5 epochs multi label)} 
& \textbf{Binary + Multi-label Feedback}
% & \textbf{BLIP (5 epoch binary +5 epochs multi label) \ryan{need better name}}
% , which the name can be described in text}} 
& 0.25B & 0 & 0 & 0 & 0 & 0 &  \textbf{0.156} &  0.019 & 0.0  & 0.0 & 0.148 \\ 
% & 0.25B & 0 & 0 & 0 & 0 & 0 &  \textbf{0.156} &  0.0191 & 0.0  & 0.0 & 0.1484 \\ 
% & \textbf{BLIP with Multi-labeled feedback (bad/neutral/good)} & 0.25B & 0 & 0 & 0 & 0 & 0 &  0.151 &  0.01747 & 0.0  & 0.0 & 0.1438 \\ 
% & \textbf{Ours-BLIP-RLHF} 

\bottomrule
\end{tabularx}
% \vspace{-1mm}
% \vspace{-2mm}
% \vspace{-2mm}
\caption{%
Results with multi-labeled human feedback.
% \todo{Fix table captions, for NeurIPS I think need to be on top of table, not bottom}
}
\label{table:results-comparison-multihf}
\end{table}





\begin{table}[b!]
\centering
% \vspace{-2mm}
% \caption{%
% Results with different human feedback metrics (BLIP-RLHF).
% }
% \label{table:results-comparison-metrics}
\renewcommand{\arraystretch}{1.1} 
\setlength{\tabcolsep}{6.9pt} 
\small
% \footnotesize
% \scriptsize
%\begin{tabularx}{1.0\linewidth}{l @{}c HH HH cc cc cccc}
\begin{tabularx}{0.6\linewidth}{l l H HH HH Hc cH Hccc}
\toprule
% & 
% % \multirow{2}{*}{\sc \# Trainable} 
% &
% \multicolumn{2}{c}{ROUGE-1} & 
% \multicolumn{2}{c}{\sc ROUGE-2} &
% % &&&&
% \multicolumn{2}{c}{\sc ROUGE-L} & \\
% \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
&
% \textsc{Human Feedback Model} 
& 
% \textsc{Parameters} & 
\textbf{\#Params} & 
R@1 & \sc Norm. & %R@1 & 
R@2 & \sc Norm. & %R@2 & 
R@L & 
% \sc Norm. & %R@L &
\textbf{ROUGE-L} &
\textbf{BLEU} & 
\textbf{CIDEr} & 
\textbf{SPICE} &
\textbf{METEOR} &
\\ \midrule

& \textbf{Helpfulness} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.1520 & 0.0186 & TODO &  0 & 0.1450 \\ 
% & \textbf{Helpfulness} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.152 & 0.019 & TODO &  0 & 0.145 \\ 
& \textbf{Takeaway} & 0.25B & 0 & 0 & 0 & 0 & 0 &   0.1676 &  0.0230 & 0.000  & 0 & 0.1598 \\ 
& \textbf{Visual} & 0.25B & 0 & 0 & 0 & 0 & 0 &  0.1678 &  0.0230 & 0.0  & 0.0 & 0.1595 \\ 
& \textbf{OCR} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.1654 & 0.0223 & TODO &  0 & 0.1565 \\ 

% \midrule
% & \textbf{Helpfulness} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.152 & 0.019 & TODO &  0 & 0.145 \\ 
% & \textbf{Takeaway} & 0.25B & 0 & 0 & 0 & 0 & 0 &   0.168 &  0.023 & 0.000  & 0 & 0.160 \\ 
% & \textbf{Visual} & 0.25B & 0 & 0 & 0 & 0 & 0 &  0.168 &  0.023 & 0.0  & 0.0 & 0.160 \\ 
% & \textbf{OCR} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.165 & 0.022 & TODO &  0 & 0.157 \\ 

\bottomrule
\end{tabularx}
% \vspace{3mm}
% \vspace{-2mm}
% \vspace{-2mm}
\caption{%
Results with different human feedback metrics (BLIP-RLHF).
}
\label{table:results-comparison-metrics}
\end{table}






\begin{table}%[t!]
\centering
\renewcommand{\arraystretch}{1.1} 
\setlength{\tabcolsep}{6.9pt} 
\small
% \footnotesize
% \scriptsize
%\begin{tabularx}{1.0\linewidth}{l @{}c HH HH cc cc cccc}
\begin{tabularx}{0.6\linewidth}{l l H HH HH Hc cH Hccc}
\toprule
% & 
% % \multirow{2}{*}{\sc \# Trainable} 
% &
% \multicolumn{2}{c}{ROUGE-1} & 
% \multicolumn{2}{c}{\sc ROUGE-2} &
% % &&&&
% \multicolumn{2}{c}{\sc ROUGE-L} & \\
% \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8}
&
% \textsc{Human Feedback Model} 
& 
% \textsc{Parameters} & 
\textbf{\#Params} & 
R@1 & \sc Norm. & %R@1 & 
R@2 & \sc Norm. & %R@2 & 
R@L & 
% \sc Norm. & %R@L &
\textbf{ROUGE-L} &
\textbf{BLEU} & 
\textbf{CIDEr} & 
\textbf{SPICE} &
\textbf{METEOR} &
\\ \midrule

& \textbf{BERT} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.1565 & 0.01927 & TODO &  0 & 0.1473 \\ 
% & \textbf{Helpfulness} & 0.25B & 0 & 0 & 0 & 0 & 0 & 0.152 & 0.019 & TODO &  0 & 0.145 \\ 
& \textbf{SciBERT} & 0.25B & 0 & 0 & 0 & 0 & 0 &   0.1577 &  0.02010 & 0.000  & 0 & 0.1509 \\ 
& \textbf{BLIP} & 0.25B & 0 & 0 & 0 & 0 & 0 &  0.1573 &  0.01977 & 0.0  & 0.0 & 0.1494 \\

\bottomrule
\end{tabularx}
% \vspace{-3mm}
% \vspace{2mm}
\caption{%
Results with different embedding models for the human-feedback model.
}
\label{table:results-comparison-diff-embedding-models}
\end{table}


